Symbol-based residual certification of reduced and neural surrogates for tempered-fractional CGMY pricing

We certify reduced and neural approximations of European-put price trajectories under the Carr--Geman--Madan--Yor model by residual bounds for the spline Galerkin discretisation of the tempered-fractional pricing equation. The Galerkin matrices are Toeplitz sections of an explicit periodised Fourier symbol; summing the alias series to a stated tail makes the assembled system exact to $10^{-8}$. A L\'evy--Khintchine argument gives the parameter-explicit bound $\lambda_{\min}(S_I)\ge r\,m_{\min}$ for the symmetric part, valid for $Y\in(0,2)\setminus\{1\}$, replacing numerical spectral estimates. A banded comparison norm built from the mass and stiffness symbols yields a rigorous certificate at $O(N)$ cost with explicit effectivity, and empirical interpolation of the symbol makes the operator affine in about 36 terms with a rigorous error transfer, so a reduced model is certified at a cost independent of $N$; a three-stage rule escalates to the full-order bounds only when needed. At the resolution that prices the whole parameter box to one cent ($N=1024$), the full-order certificate costs 6% of a direct solve, and the certified POD--Galerkin model of rank 80 costs 3% of it and settles 99.8% of $10^4$ queries without touching the full space. No false accept occurs on any query with a reference solution (150 inside the parameter box, 264 outside), and outside the box the certificate accepts 193 of the 210 queries on which the reduced model is still within one cent. The neural reduced models trained here miss the one-cent tolerance by a factor of at least 46; the certificate detects this at every query in a few milliseconds and explains it as a trade-off between temporal smoothness and coefficient accuracy. A residual certificate for the American put is proved as an outlook.

==> xref_main.tex <==
% Cross-references to the main article, frozen from its compiled .aux.
\newlabel{sec:introduction}{{1}{1}{Introduction}{}{}}
\newlabel{sec:introduction@cref}{{[section][1][]1}{[1][1][]1}}
\newlabel{sec:model}{{2}{2}{CGMY model and constrained discretisation}{}{}}
\newlabel{sec:model@cref}{{[section][2][]2}{[1][2][]2}}
\newlabel{sec:galerkin}{{2}{2}{CGMY model and constrained discretisation}{}{}}
\newlabel{sec:galerkin@cref}{{[section][2][]2}{[1][2][]2}}
\newlabel{ssec:operator}{{2.1}{2}{CGMY backward operator}{}{}}
\newlabel{ssec:operator@cref}{{[subsection][1][2]2.1}{[1][2][]2}}
\newlabel{eq:cgmy-parameters}{{2.1}{2}{CGMY backward operator}{}{}}
\newlabel{eq:cgmy-parameters@cref}{{[equation][1][2]2.1}{[1][2][]2}}
\newlabel{tab:notation}{{1.1}{3}{Notation}{}{}}
\newlabel{tab:notation@cref}{{[table][1][1]1.1}{[1][2][]3}}
\newlabel{eq:martingale-correction}{{2.2}{3}{CGMY backward operator}{}{}}
\newlabel{eq:martingale-correction@cref}{{[equation][2][2]2.2}{[1][2][]3}}
\newlabel{eq:lambda0}{{2.3}{3}{CGMY backward operator}{}{}}
\newlabel{eq:lambda0@cref}{{[equation][3][2]2.3}{[1][3][]3}}
\newlabel{eq:tempered-ops}{{2.4}{3}{CGMY backward operator}{}{}}
\newlabel{eq:tempered-ops@cref}{{[equation][4][2]2.4}{[1][3][]3}}
\newlabel{eq:cgmy-operator}{{2.5}{3}{CGMY backward operator}{}{}}
\newlabel{eq:cgmy-operator@cref}{{[equation][5][2]2.5}{[1][3][]3}}
\newlabel{eq:pricing-pide}{{2.6}{3}{CGMY backward operator}{}{}}
\newlabel{eq:pricing-pide@cref}{{[equation][6][2]2.6}{[1][3][]3}}
\newlabel{eq:symbol}{{2.7}{3}{CGMY backward operator}{}{}}
\newlabel{eq:symbol@cref}{{[equation][7][2]2.7}{[1][3][]3}}
\newlabel{ssec:family}{{2.2}{3}{Parameter family and exterior data}{}{}}
\newlabel{ssec:family@cref}{{[subsection][2][2]2.2}{[1][3][]3}}
\newlabel{ssec:finite-domain}{{2.2}{3}{Parameter family and exterior data}{}{}}
\newlabel{ssec:finite-domain@cref}{{[subsection][2][2]2.2}{[1][3][]3}}
\newlabel{eq:parameter-set}{{2.8}{3}{Parameter family and exterior data}{}{}}
\newlabel{eq:parameter-set@cref}{{[equation][8][2]2.8}{[1][3][]3}}
\newlabel{eq:numerical-box}{{2.9}{4}{Parameter family and exterior data}{}{}}
\newlabel{eq:numerical-box@cref}{{[equation][9][2]2.9}{[1][3][]4}}
\newlabel{eq:energy-space}{{2.10}{4}{Parameter family and exterior data}{}{}}
\newlabel{eq:energy-space@cref}{{[equation][10][2]2.10}{[1][4][]4}}
\newlabel{eq:HMG-norm}{{2.11}{4}{Parameter family and exterior data}{}{}}
\newlabel{eq:HMG-norm@cref}{{[equation][11][2]2.11}{[1][4][]4}}
\newlabel{eq:weak-problem}{{2.12}{4}{Parameter family and exterior data}{}{}}
\newlabel{eq:weak-problem@cref}{{[equation][12][2]2.12}{[1][4][]4}}
\newlabel{eq:lifting-functional}{{2.13}{4}{Parameter family and exterior data}{}{}}
\newlabel{eq:lifting-functional@cref}{{[equation][13][2]2.13}{[1][4][]4}}
\newlabel{ssec:uniform}{{2.3}{4}{Uniform variational stability}{}{}}
\newlabel{ssec:uniform@cref}{{[subsection][3][2]2.3}{[1][4][]4}}
\newlabel{thm:uniform-coercivity}{{2.1}{4}{Uniform variational stability}{}{}}
\newlabel{thm:uniform-coercivity@cref}{{[theorem][1][2]2.1}{[1][4][]4}}
\newlabel{eq:uniform-coercivity}{{2.14}{4}{Uniform variational stability}{}{}}
\newlabel{eq:uniform-coercivity@cref}{{[equation][14][2]2.14}{[1][4][]4}}
\newlabel{rem:coercivity}{{2.2}{4}{Uniform variational stability}{}{}}
\newlabel{rem:coercivity@cref}{{[remark][2][2]2.2}{[1][4][]4}}
\newlabel{ssec:spline-space}{{2.4}{5}{Spline space and assembly}{}{}}
\newlabel{ssec:spline-space@cref}{{[subsection][4][2]2.4}{[1][4][]5}}
\newlabel{eq:Vh}{{2.15}{5}{Spline space and assembly}{}{}}
\newlabel{eq:Vh@cref}{{[equation][15][2]2.15}{[1][5][]5}}
\newlabel{eq:matrices}{{2.16}{5}{Spline space and assembly}{}{}}
\newlabel{eq:matrices@cref}{{[equation][16][2]2.16}{[1][5][]5}}
\newlabel{eq:Ah}{{2.17}{5}{Spline space and assembly}{}{}}
\newlabel{eq:Ah@cref}{{[equation][17][2]2.17}{[1][5][]5}}
\newlabel{eq:toeplitz-blocks}{{2.18}{5}{Spline space and assembly}{}{}}
\newlabel{eq:toeplitz-blocks@cref}{{[equation][18][2]2.18}{[1][5][]5}}
\newlabel{eq:semidiscrete-system}{{2.19}{5}{Spline space and assembly}{}{}}
\newlabel{eq:semidiscrete-system@cref}{{[equation][19][2]2.19}{[1][5][]5}}
\newlabel{ssec:assembly}{{2.5}{5}{Exact assembly from the periodised symbol}{}{}}
\newlabel{ssec:assembly@cref}{{[subsection][5][2]2.5}{[1][5][]5}}
\newlabel{lem:periodisation}{{2.3}{5}{Exact assembly from the periodised symbol}{}{}}
\newlabel{lem:periodisation@cref}{{[lemma][3][2]2.3}{[1][5][]5}}
\newlabel{eq:periodised}{{2.20}{5}{Exact assembly from the periodised symbol}{}{}}
\newlabel{eq:periodised@cref}{{[equation][20][2]2.20}{[1][5][]5}}
\newlabel{lem:tail}{{2.4}{6}{Exact assembly from the periodised symbol}{}{}}
\newlabel{lem:tail@cref}{{[lemma][4][2]2.4}{[1][6][]6}}
\newlabel{eq:tail}{{2.21}{6}{Exact assembly from the periodised symbol}{}{}}
\newlabel{eq:tail@cref}{{[equation][21][2]2.21}{[1][6][]6}}
\newlabel{lem:toeplitz}{{2.5}{6}{Exact assembly from the periodised symbol}{}{}}
\newlabel{lem:toeplitz@cref}{{[lemma][5][2]2.5}{[1][6][]6}}
\newlabel{ssec:constrained-system}{{2.6}{7}{Prescribed coefficients and the free system}{}{}}
\newlabel{ssec:constrained-system@cref}{{[subsection][6][2]2.6}{[1][7][]7}}
\newlabel{eq:constrained-cn}{{2.22}{7}{Prescribed coefficients and the free system}{}{}}
\newlabel{eq:constrained-cn@cref}{{[equation][22][2]2.22}{[1][7][]7}}
\newlabel{eq:constrained-residual}{{2.23}{7}{Prescribed coefficients and the free system}{}{}}
\newlabel{eq:constrained-residual@cref}{{[equation][23][2]2.23}{[1][7][]7}}
\newlabel{eq:sections}{{2.24}{7}{Prescribed coefficients and the free system}{}{}}
\newlabel{eq:sections@cref}{{[equation][24][2]2.24}{[1][7][]7}}
\newlabel{ssec:reference-time}{{2.7}{7}{Time discretisation and error target}{}{}}
\newlabel{ssec:reference-time@cref}{{[subsection][7][2]2.7}{[1][7][]7}}
\newlabel{ssec:deterministic-error}{{2.7}{7}{Time discretisation and error target}{}{}}
\newlabel{ssec:deterministic-error@cref}{{[subsection][7][2]2.7}{[1][7][]7}}
\newlabel{ssec:lifting-cancels}{{2.7}{7}{Time discretisation and error target}{}{}}
\newlabel{ssec:lifting-cancels@cref}{{[subsection][7][2]2.7}{[1][7][]7}}
\newlabel{eq:cn-reference}{{2.25}{7}{Time discretisation and error target}{}{}}
\newlabel{eq:cn-reference@cref}{{[equation][25][2]2.25}{[1][7][]7}}
\newlabel{eq:total-error-split}{{2.26}{7}{Time discretisation and error target}{}{}}
\newlabel{eq:total-error-split@cref}{{[equation][26][2]2.26}{[1][7][]7}}
\newlabel{ssec:spectral}{{2.8}{8}{Spectral lower bound}{}{}}
\newlabel{ssec:spectral@cref}{{[subsection][8][2]2.8}{[1][8][]8}}
\newlabel{lem:LK}{{2.6}{8}{Spectral lower bound}{}{}}
\newlabel{lem:LK@cref}{{[lemma][6][2]2.6}{[1][8][]8}}
\newlabel{thm:spectral}{{2.7}{8}{Spectral lower bound}{}{}}
\newlabel{thm:spectral@cref}{{[theorem][7][2]2.7}{[1][8][]8}}
\newlabel{eq:spectral}{{2.27}{8}{Spectral lower bound}{}{}}
\newlabel{eq:spectral@cref}{{[equation][27][2]2.27}{[1][8][]8}}
\newlabel{rem:compression}{{2.8}{8}{Spectral lower bound}{}{}}
\newlabel{rem:compression@cref}{{[remark][8][2]2.8}{[1][8][]8}}
\newlabel{sec:certificate}{{3}{9}{Residual certification and tolerance-controlled correction}{}{}}
\newlabel{sec:certificate@cref}{{[section][3][]3}{[1][9][]9}}
\newlabel{sec:pcc}{{3}{9}{Residual certification and tolerance-controlled correction}{}{}}
\newlabel{sec:pcc@cref}{{[section][3][]3}{[1][9][]9}}
\newlabel{ssec:riesz}{{3.1}{9}{Energy norm and Crank--Nicolson bound}{}{}}
\newlabel{ssec:riesz@cref}{{[subsection][1][3]3.1}{[1][9][]9}}
\newlabel{ssec:cn-certificate}{{3.1}{9}{Energy norm and Crank--Nicolson bound}{}{}}
\newlabel{ssec:cn-certificate@cref}{{[subsection][1][3]3.1}{[1][9][]9}}
\newlabel{eq:Sh}{{3.1}{9}{Energy norm and Crank--Nicolson bound}{}{}}
\newlabel{eq:Sh@cref}{{[equation][1][3]3.1}{[1][9][]9}}
\newlabel{eq:cn-residual}{{3.2}{9}{Energy norm and Crank--Nicolson bound}{}{}}
\newlabel{eq:cn-residual@cref}{{[equation][2][3]3.2}{[1][9][]9}}
\newlabel{eq:discrete-error-equation}{{3.3}{9}{Energy norm and Crank--Nicolson bound}{}{}}
\newlabel{eq:discrete-error-equation@cref}{{[equation][3][3]3.3}{[1][9][]9}}
\newlabel{thm:fully-discrete-certificate}{{3.1}{9}{Energy norm and Crank--Nicolson bound}{}{}}
\newlabel{thm:fully-discrete-certificate@cref}{{[theorem][1][3]3.1}{[1][9][]9}}
\newlabel{eq:fully-discrete-certificate}{{3.4}{9}{Energy norm and Crank--Nicolson bound}{}{}}
\newlabel{eq:fully-discrete-certificate@cref}{{[equation][4][3]3.4}{[1][9][]9}}
\newlabel{eq:sharp-estimator}{{3.5}{9}{Energy norm and Crank--Nicolson bound}{}{}}
\newlabel{eq:sharp-estimator@cref}{{[equation][5][3]3.5}{[1][9][]9}}
\newlabel{eq:sharp-L2}{{3.6}{9}{Energy norm and Crank--Nicolson bound}{}{}}
\newlabel{eq:sharp-L2@cref}{{[equation][6][3]3.6}{[1][9][]9}}
\newlabel{ssec:guaranteed}{{3.2}{10}{Upper bounds from incomplete Riesz solves}{}{}}
\newlabel{ssec:guaranteed@cref}{{[subsection][2][3]3.2}{[1][10][]10}}
\newlabel{eq:alpha-lb}{{3.7}{10}{Upper bounds from incomplete Riesz solves}{}{}}
\newlabel{eq:alpha-lb@cref}{{[equation][7][3]3.7}{[1][10][]10}}
\newlabel{lem:guaranteed}{{3.2}{10}{Upper bounds from incomplete Riesz solves}{}{}}
\newlabel{lem:guaranteed@cref}{{[lemma][2][3]3.2}{[1][10][]10}}
\newlabel{eq:riesz-bracket-def}{{3.8}{10}{Upper bounds from incomplete Riesz solves}{}{}}
\newlabel{eq:riesz-bracket-def@cref}{{[equation][8][3]3.8}{[1][10][]10}}
\newlabel{cor:guaranteed}{{3.3}{10}{Upper bounds from incomplete Riesz solves}{}{}}
\newlabel{cor:guaranteed@cref}{{[corollary][3][3]3.3}{[1][10][]10}}
\newlabel{eq:guaranteed-estimator}{{3.9}{10}{Upper bounds from incomplete Riesz solves}{}{}}
\newlabel{eq:guaranteed-estimator@cref}{{[equation][9][3]3.9}{[1][10][]10}}
\newlabel{rem:arithmetic-scope}{{3.4}{10}{Upper bounds from incomplete Riesz solves}{}{}}
\newlabel{rem:arithmetic-scope@cref}{{[remark][4][3]3.4}{[1][10][]10}}
\newlabel{ssec:comparison}{{3.3}{10}{A banded comparison norm}{}{}}
\newlabel{ssec:comparison@cref}{{[subsection][3][3]3.3}{[1][10][]10}}
\newlabel{thm:comparison}{{3.5}{11}{A banded comparison norm}{}{}}
\newlabel{thm:comparison@cref}{{[theorem][5][3]3.5}{[1][10][]11}}
\newlabel{eq:comparison}{{3.10}{11}{A banded comparison norm}{}{}}
\newlabel{eq:comparison@cref}{{[equation][10][3]3.10}{[1][11][]11}}
\newlabel{cor:cheap}{{3.6}{11}{A banded comparison norm}{}{}}
\newlabel{cor:cheap@cref}{{[corollary][6][3]3.6}{[1][11][]11}}
\newlabel{prop:twostage}{{3.7}{11}{A banded comparison norm}{}{}}
\newlabel{prop:twostage@cref}{{[proposition][7][3]3.7}{[1][11][]11}}
\newlabel{prop:threestage}{{3.8}{11}{A banded comparison norm}{}{}}
\newlabel{prop:threestage@cref}{{[proposition][8][3]3.8}{[1][11][]11}}
\newlabel{ssec:efficiency}{{3.4}{12}{Efficiency and spot-price bounds}{}{}}
\newlabel{ssec:efficiency@cref}{{[subsection][4][3]3.4}{[1][12][]12}}
\newlabel{ssec:greeks-cert}{{3.4}{12}{Efficiency and spot-price bounds}{}{}}
\newlabel{ssec:greeks-cert@cref}{{[subsection][4][3]3.4}{[1][12][]12}}
\newlabel{eq:kappa-def}{{3.11}{12}{Efficiency and spot-price bounds}{}{}}
\newlabel{eq:kappa-def@cref}{{[equation][11][3]3.11}{[1][12][]12}}
\newlabel{thm:efficiency}{{3.9}{12}{Efficiency and spot-price bounds}{}{}}
\newlabel{thm:efficiency@cref}{{[theorem][9][3]3.9}{[1][12][]12}}
\newlabel{eq:efficiency}{{3.12}{12}{Efficiency and spot-price bounds}{}{}}
\newlabel{eq:efficiency@cref}{{[equation][12][3]3.12}{[1][12][]12}}
\newlabel{eq:gamma-infty}{{3.13}{12}{Efficiency and spot-price bounds}{}{}}
\newlabel{eq:gamma-infty@cref}{{[equation][13][3]3.13}{[1][12][]12}}
\newlabel{alg:pcc}{{3.1}{13}{Tolerance-checked online rule (the three-stage rule of Proposition~\ref {prop:threestage} followed by correction). The status names are those used in the tables of Section~\ref {sec:numerics}}{}{}}
\newlabel{alg:pcc@cref}{{[figure][1][3]3.1}{[1][12][]13}}
\newlabel{ssec:algorithm}{{3.5}{13}{Tolerance-controlled prediction and correction}{}{}}
\newlabel{ssec:algorithm@cref}{{[subsection][5][3]3.5}{[1][12][]13}}
\newlabel{ssec:two-stage}{{3.5}{13}{Tolerance-controlled prediction and correction}{}{}}
\newlabel{ssec:two-stage@cref}{{[subsection][5][3]3.5}{[1][12][]13}}
\newlabel{ssec:correction}{{3.5}{13}{Tolerance-controlled prediction and correction}{}{}}
\newlabel{ssec:correction@cref}{{[subsection][5][3]3.5}{[1][12][]13}}
\newlabel{prop:two-stage}{{3.10}{13}{Tolerance-controlled prediction and correction}{}{}}
\newlabel{prop:two-stage@cref}{{[proposition][10][3]3.10}{[1][13][]13}}
\newlabel{eq:soundness}{{3.14}{13}{Tolerance-controlled prediction and correction}{}{}}
\newlabel{eq:soundness@cref}{{[equation][14][3]3.14}{[1][13][]13}}
\newlabel{eq:correction-step}{{3.15}{13}{Tolerance-controlled prediction and correction}{}{}}
\newlabel{eq:correction-step@cref}{{[equation][15][3]3.15}{[1][13][]13}}
\newlabel{sec:affine}{{4}{14}{Affine structure and surrogate candidates}{}{}}
\newlabel{sec:affine@cref}{{[section][4][]4}{[1][13][]14}}
\newlabel{sec:operator}{{4}{14}{Affine structure and surrogate candidates}{}{}}
\newlabel{sec:operator@cref}{{[section][4][]4}{[1][13][]14}}
\newlabel{ssec:eim}{{4.1}{14}{Affine decomposition of the fractional blocks}{}{}}
\newlabel{ssec:eim@cref}{{[subsection][1][4]4.1}{[1][14][]14}}
\newlabel{eq:affine-split}{{4.1}{14}{Affine decomposition of the fractional blocks}{}{}}
\newlabel{eq:affine-split@cref}{{[equation][1][4]4.1}{[1][14][]14}}
\newlabel{lem:eim}{{4.1}{14}{Affine decomposition of the fractional blocks}{}{}}
\newlabel{lem:eim@cref}{{[lemma][1][4]4.1}{[1][14][]14}}
\newlabel{fig:eim}{{4.1}{15}{Empirical interpolation of the fractional symbol family. (a) Relative sup-norm error on $1000$ Sobol test parameters (solid) and normalised singular values of the $16^3$ training snapshots (dotted), $N=64$--$1024$. (b) Rank $Q$ needed for a given test tolerance; the curves for $N=512$ and $N=1024$ coincide. The operational $Q$ additionally satisfies the operator-norm check (one extra term at $N=64$)}{}{}}
\newlabel{fig:eim@cref}{{[figure][1][4]4.1}{[1][14][]15}}
\newlabel{thm:eim-cert}{{4.2}{15}{Affine decomposition of the fractional blocks}{}{}}
\newlabel{thm:eim-cert@cref}{{[theorem][2][4]4.2}{[1][15][]15}}
\newlabel{rem:reduced-online}{{4.3}{15}{Affine decomposition of the fractional blocks}{}{}}
\newlabel{rem:reduced-online@cref}{{[remark][3][4]4.3}{[1][15][]15}}
\newlabel{ssec:target}{{4.2}{16}{Candidates, initial target and training objective}{}{}}
\newlabel{ssec:target@cref}{{[subsection][2][4]4.2}{[1][16][]16}}
\newlabel{ssec:architectures}{{4.2}{16}{Candidates, initial target and training objective}{}{}}
\newlabel{ssec:architectures@cref}{{[subsection][2][4]4.2}{[1][16][]16}}
\newlabel{ssec:exact-ic}{{4.2}{16}{Candidates, initial target and training objective}{}{}}
\newlabel{ssec:exact-ic@cref}{{[subsection][2][4]4.2}{[1][16][]16}}
\newlabel{ssec:losses}{{4.2}{16}{Candidates, initial target and training objective}{}{}}
\newlabel{ssec:losses@cref}{{[subsection][2][4]4.2}{[1][16][]16}}
\newlabel{sec:data}{{4.2}{16}{Candidates, initial target and training objective}{}{}}
\newlabel{sec:data@cref}{{[subsection][2][4]4.2}{[1][16][]16}}
\newlabel{eq:residual-loss}{{4.2}{16}{Candidates, initial target and training objective}{}{}}
\newlabel{eq:residual-loss@cref}{{[equation][2][4]4.2}{[1][16][]16}}
\newlabel{ssec:pod-construction}{{4.3}{16}{Mass-weighted POD trajectories}{}{}}
\newlabel{ssec:pod-construction@cref}{{[subsection][3][4]4.3}{[1][16][]16}}
\newlabel{eq:repaired-pod-cn}{{4.3}{17}{Mass-weighted POD trajectories}{}{}}
\newlabel{eq:repaired-pod-cn@cref}{{[equation][3][4]4.3}{[1][16][]17}}
\newlabel{ssec:cost}{{4.4}{18}{Cost model}{}{}}
\newlabel{ssec:cost@cref}{{[subsection][4][4]4.4}{[1][18][]18}}
\newlabel{sec:numerics}{{5}{18}{Numerical evaluation}{}{}}
\newlabel{sec:numerics@cref}{{[section][5][]5}{[1][18][]18}}
\newlabel{ssec:design}{{5.1}{18}{Experimental design}{}{}}
\newlabel{ssec:design@cref}{{[subsection][1][5]5.1}{[1][18][]18}}
\newlabel{tab:populations}{{5.1}{18}{Experimental design}{}{}}
\newlabel{tab:populations@cref}{{[subsection][1][5]5.1}{[1][18][]18}}
\newlabel{ssec:verification}{{5.2}{18}{Verification of the assembly, the bounds and the solvers}{}{}}
\newlabel{ssec:verification@cref}{{[subsection][2][5]5.2}{[1][18][]18}}
\newlabel{ssec:e0-assembly}{{5.2}{18}{Verification of the assembly, the bounds and the solvers}{}{}}
\newlabel{ssec:e0-assembly@cref}{{[subsection][2][5]5.2}{[1][18][]18}}
\newlabel{ssec:e0-spectral}{{5.2}{18}{Verification of the assembly, the bounds and the solvers}{}{}}
\newlabel{ssec:e0-spectral@cref}{{[subsection][2][5]5.2}{[1][18][]18}}
\newlabel{ssec:e0-riesz}{{5.2}{18}{Verification of the assembly, the bounds and the solvers}{}{}}
\newlabel{ssec:e0-riesz@cref}{{[subsection][2][5]5.2}{[1][18][]18}}
\newlabel{ssec:e0-initial}{{5.2}{18}{Verification of the assembly, the bounds and the solvers}{}{}}
\newlabel{ssec:e0-initial@cref}{{[subsection][2][5]5.2}{[1][18][]18}}
\newlabel{ssec:calibration}{{5.3}{19}{Resolution and tolerance calibration}{}{}}
\newlabel{ssec:calibration@cref}{{[subsection][3][5]5.3}{[1][19][]19}}
\newlabel{tab:budget}{{5.1}{19}{Resolution and tolerance calibration: maximum price error $\max |V_h(T,S)-V_{\mathrm {COS}}|$ over the 30 price-diagnostic queries and the two box corners, spots $S\in \{0.8,\dots ,1.2\}\mathcal K$; COS with 8192 modes, range parameter 30. $\varepsilon _N=\tau _\$/\max _s\beta _I(x_s)$ with $\tau _\$=1$ cent}{}{}}
\newlabel{tab:budget@cref}{{[table][1][5]5.1}{[1][19][]19}}
\newlabel{ssec:e1}{{5.4}{19}{Reduced model and neural candidates}{}{}}
\newlabel{ssec:e1@cref}{{[subsection][4][5]5.4}{[1][19][]19}}
\newlabel{ssec:pod-results}{{5.4}{19}{Reduced model and neural candidates}{}{}}
\newlabel{ssec:pod-results@cref}{{[subsection][4][5]5.4}{[1][19][]19}}
\newlabel{tab:pod-ranks}{{5.2}{20}{POD--Galerkin candidates on the 30 validation queries at the production configuration ($N=1024$, $N_T=240$, $Q$ matched to $\varepsilon $): median maximum-in-time mass-norm error against the direct solution, median effectivity (bound/error) of the three certificates, queries accepted at $\varepsilon _N=1.18\times 10^{-3}$ under each certificate, and the stage at which the three-stage rule of Proposition~\ref {prop:threestage} settles the query (reduced accept / cheap reject / banded accept / exact accept / exact reject). Basis from 800 training trajectories; the 4000-trajectory basis gives the same picture (Section~\ref {ssec:e1}). No false accepts occur under any certificate at any tolerance of the sweep}{}{}}
\newlabel{tab:pod-ranks@cref}{{[table][2][5]5.2}{[1][19][]20}}
\newlabel{fig:acceptance}{{5.1}{20}{Top: accepted fraction of the 30 validation queries as a function of the tolerance $\varepsilon $ (dashed line: $\varepsilon _N$) for POD--Galerkin candidates of rank $48$--$80$ and the two best POD-NN checkpoints, under the reduced online, banded full-order and exact full-order certificates. Bottom: the stage at which the three-stage rule of Proposition~\ref {prop:threestage} settles each query at $\varepsilon _N$, per rank}{}{}}
\newlabel{fig:acceptance@cref}{{[figure][1][5]5.1}{[1][19][]20}}
\newlabel{ssec:benchmark}{{5.5}{21}{Matched benchmark and cost under refinement}{}{}}
\newlabel{ssec:benchmark@cref}{{[subsection][5][5]5.5}{[1][21][]21}}
\newlabel{ssec:scaling-results}{{5.5}{21}{Matched benchmark and cost under refinement}{}{}}
\newlabel{ssec:scaling-results@cref}{{[subsection][5][5]5.5}{[1][21][]21}}
\newlabel{fig:benchmark}{{5.2}{22}{Top: time ratio to the uncertified direct solve on the 120 benchmark queries at $\varepsilon =0.3\varepsilon _N$, $\varepsilon _N$, $3\varepsilon _N$ (geometric means, $95\%$ query-bootstrap intervals, reusable setup). Bottom left: direct solve and banded full-order certificate per query as functions of $N$ (20 benchmark queries, $N_T=240$), with the reduced online certificate at $r=64$ and $80$, which does not depend on $N$. Bottom right: the certificate as a fraction of the solve, $4.5$--$5.6\%$ for $N=64$--$4096$}{}{}}
\newlabel{fig:benchmark@cref}{{[figure][2][5]5.2}{[1][21][]22}}
\newlabel{tab:benchmark}{{5.3}{22}{Matched benchmark on the 120 benchmark queries at the production configuration (one thread, idle machine, reusable setup, five repetitions): geometric-mean time ratio to the uncertified direct solve with 95\% query-bootstrap interval, three-stage outcome (reduced accept / cheap reject / banded or exact accept / corrected), and false accepts. The direct solve takes $259$~ms; the certificate proper is $6.0\%$ of it and $7.2\%$ with the per-query spectral data}{}{}}
\newlabel{tab:benchmark@cref}{{[table][3][5]5.3}{[1][21][]22}}
\newlabel{ssec:ood}{{5.6}{22}{Out-of-distribution detection}{}{}}
\newlabel{ssec:ood@cref}{{[subsection][6][5]5.6}{[1][21][]22}}
\newlabel{tab:ood}{{5.4}{23}{Out-of-distribution study: 264 queries outside the parameter box (200 Sobol points in the shells $C\in [1,2]$, $Y\in [0.9,1.1)\cup (1.8,1.95]$, $G\in [0.5,1)$, $M\in [9,15]$, and 64 vertices of the extended box) at the production configuration. Top: queries on which the candidate's true error is below $\varepsilon _N$ (``works''), queries the exact certificate accepts (``certified''), and precision of two rules as detectors of ``true error $>\varepsilon _N$'': the certificate (recall 1 by theorem) and the naive rule that rejects every query outside the training box (recall 1, but it discards every working query). Bottom: POD--Galerkin $r=80$ by shell (a query leaving the box in several coordinates counts in each), with the median true error and the median EIM error $\varepsilon _Q$ (inside the box: $1.7\times 10^{-9}$)}{}{}}
\newlabel{tab:ood@cref}{{[table][4][5]5.4}{[1][22][]23}}
\newlabel{fig:ood}{{5.3}{23}{Certified bound against true error for the 264 out-of-box queries and the 30 validation queries (POD--Galerkin $r=64$ and $80$, space--time POD-NN), under the three certificates; the lines mark $\varepsilon _N$ and bound $=$ error}{}{}}
\newlabel{fig:ood@cref}{{[figure][3][5]5.3}{[1][22][]23}}
\newlabel{ssec:multiquery}{{5.7}{23}{Multi-query cost and amortisation}{}{}}
\newlabel{ssec:multiquery@cref}{{[subsection][7][5]5.7}{[1][23][]23}}
\newlabel{fig:online-time}{{5.4}{24}{Online time per query of the reduced model at the production configuration (one thread, idle machine): reduced solve, reduced online certificate, and the three-stage total at $\varepsilon _N$, against the uncertified direct solve (dashed: cold-start and reusable-setup medians of the benchmark of Section~\ref {ssec:benchmark})}{}{}}
\newlabel{fig:online-time@cref}{{[figure][4][5]5.4}{[1][23][]24}}
\newlabel{fig:amortisation}{{5.5}{24}{Cumulative wall time, offline cost included, against the number of queries at the production configuration (one thread); dots mark the break-even with the uncertified direct solver}{}{}}
\newlabel{fig:amortisation@cref}{{[figure][5][5]5.5}{[1][23][]24}}
\newlabel{ssec:archive}{{5.8}{24}{Reproducibility}{}{}}
\newlabel{ssec:archive@cref}{{[subsection][8][5]5.8}{[1][24][]24}}
\newlabel{sec:conclusion}{{6}{24}{Interpretation and conclusion}{}{}}
\newlabel{sec:conclusion@cref}{{[section][6][]6}{[1][24][]24}}
\newlabel{sec:discussion}{{6}{24}{Interpretation and conclusion}{}{}}
\newlabel{sec:discussion@cref}{{[section][6][]6}{[1][24][]24}}

